An Empirical Study on the Effectiveness of Large Language Models for SATD Identification and Classification

Self-Admitted Technical Debt (SATD), a concept highlighting sub-optimal choices in software development documented in code comments or other project resources, poses challenges in the maintainability and evolution of software systems. Large language models (LLMs) have demonstrated significant effectiveness across a broad range of software tasks, especially in software text generation tasks. Nonetheless, their effectiveness in tasks related to SATD is still under-researched. In this paper, we investigate the efficacy of LLMs in both identification and classification of SATD. For both tasks, we investigate the performance gain from using more recent LLMs, specifically the Flan-T5 family, across different common usage settings. Our results demonstrate that for SATD identification, all fine-tuned LLMs outperform the best existing non-LLM baseline, i.e., the CNN model, with a 4.4% to 7.2% improvement in F1 score. In the SATD classification task, while our largest fine-tuned model, Flan-T5-XL, still led in performance, the CNN model exhibited competitive results, even surpassing four of six LLMs. We also found that the largest Flan-T5 model, i.e., Flan-T5-XXL, when used with a zero-shot in-context learning (ICL) approach for SATD identification, provides competitive results with traditional approaches but performs 6.4% to 9.2% worse than fine-tuned LLMs. For SATD classification, few-shot ICL approach, incorporating examples and category descriptions in prompts, outperforms the zero-shot approach and even surpasses the fine-tuned smaller Flan-T5 models. Moreover, our experiments demonstrate that incorporating contextual information, such as surrounding code, into the SATD classification task enables larger fine-tuned LLMs to improve their performance.

==> _RQs_delete_it.tex <==
\yuan{too late, these two tasks should be introduced in the introduction and repeated in related work.}Before presenting the research questions, it is essential to define the tasks of SATD identification and classification. SATD identification is a binary classification task that determines whether a given input, such as comment text, is SATD or non-SATD. Conversely, the SATD classification task presupposes the presence of an identified SATD and aims to detect its category (e.g., Code, Defect, Design, etc.). Having clarified these tasks, let's now present our research questions.

In this section, we introduce the four research questions (RQs) that steered our empirical study, along with the underlying motivation for each question. 

\paragraph{\textbf{\rqone}}
Previous studies have explored pattern-based methods, as well as machine learning and deep learning approaches, for identifying and classifying SATD. A notable recent study by Prenner and Robbes~\citep{Prenner-2022} employed the BERT model for several classification tasks in software engineering, including SATD identification, and achieved significant improvements over traditional methods. The success of BERT in this domain, combined with the advent of more sophisticated, larger, open-source\yuan{why closed LLMs are not an option? because they are too expensive?this should be mentioned early, maybe in related work} language models like T5 and LLaMA, has inspired our investigation of their effectiveness for SATD identification and classification. Therefore, our first research question explores whether these newer and more advanced language models, known for their proficiency in text generation tasks such as summarization and translation, can also outperform BERT in the efficient identification and classification of SATD. In our experiments for RQ1, we employed the Flan-T5 models, BERT, and CodeBERT as the chosen LLMs for fine-tuning and compared their results with non-LLM baselines. The rationale for selecting these models is presented in Section~\ref{subsec:selected_llm}.

\paragraph{\textbf{\rqtwo}}
While RQ1 focuses on fine-tuning pre-trained models, this research question explores whether ICL using a larger LLM can surpass the performance of smaller models that have been fine-tuned for SATD identification and classification. ICL is notably cost-effective during the training phase, just requiring prompt engineering\yuan{please ensure we mention prompt engineering and explain it in the introduction when we introduce ICL}, making it an appealing approach, especially when training data is limited. To assess the efficacy of the ICL approach, we utilize Flan-T5-xxl with 11.1B parameters, which is approximately four times larger than the biggest model fine-tuned in this study, namely, Flan-T5-xl with 2.85B parameters.

\paragraph{\textbf{\rqthree}}
In RQ1 and RQ2, the models are given only the code comments - the default setting for existing SATD identification and classification approaches. The aim of RQ3 is to explore whether including additional contexts, such as the file path, the containing method's signature, and the body of the containing method, enhances the performance of large language models in the SATD classification task. A key aspect of this investigation is determining the optimal size of the LLM required to effectively utilize this contextual data for improved results. Specifically, we want to assess whether smaller LLMs can discern patterns and relationships between the code comments and the contextual features to enhance SATD classification performance. We only investigate this question for SATD classification because the largest benchmark for SATD identification, i.e., the Maldonado dataset~\citep{Maldonado-2017} did not provide the location and contextual information for each SATD.

\paragraph{\textbf{\rqfour}}\sw{put this RQ before current RQ3.}
\sw{I guess a good motivation is that two ways to do so, 1) directly output the label, and cite some sentiment classification papers. 2) modifying the output layer. we would like to investigate which one is good. By doing so, we can provide insights for classification tasks using LLM.}
\yuan{why this is needed? not motivated}In order to employ the Flan-T5 models for SATD identification and classification, we refine their architecture by substituting the original text generation layer with a classification layer to better adapt the model for classification tasks (see Section~\ref{subsec:architecture}). To assess the impact of this architectural modification, we conduct some experiments using the original Flan-T5 models, and inputting only the comment text. 
